Irrelevant Pixels are Everywhere: Find and Exclude Them for More Efficient Computer Vision

Computer vision is often performed using Convolutional Neural Networks (CNNs). CNNs are compute-intensive and challenging to deploy on power-contrained systems such as mobile and Internet-of-Things (IoT) devices. CNNs are compute-intensive because they indiscriminately compute many features on all pixels of the input image. We observe that, given a computer vision task, images often contain pixels that are irrelevant to the task. For example, if the task is looking for cars, pixels in the sky are not very useful. Therefore, we propose that a CNN be modified to only operate on relevant pixels to save computation and energy. We propose a method to study three popular computer vision datasets, finding that 48% of pixels are irrelevant. We also propose the focused convolution to modify a CNN's convolutional layers to reject the pixels that are marked irrelevant. On an embedded device, we observe no loss in accuracy, while inference latency, energy consumption, and multiply-add count are all reduced by about 45%.

==> old-2-dataset-examination.tex <==
\section{\dif{Finding Irrelevant Pixels in Datasets}}
\label{sec:irrelevant-pixels-in-popular-datasets}
We study the COCO, PASCAL VOC, and MOTChallenge to demonstrate that irrelevant pixels are commonly found in popular computer vision datasets. \dif{These datasets contain ground truth labels (each label is a list of pixels that comprise an relevant object). We augment the ground truth with our depth mapping technique to count approximately 48\% of pixels in the datasets as irrelevant.}

\subsection{\diff{Counting Irrelevant Pixels via Depthmaps \& Ground Truth}}
\label{subsec:using-depth-maps-to-count-irrelevant-pixels}
Our study defines a dataset's relevant pixels as: \textit{all pixels that comprise the dataset ground truth objects and their associated depth levels.} In \autoref{fig:irrelevant-pixels-example}a, the ground truth pixels are represented by the red area around the shuttle buses. By adding additional pixels in the depth level (explained later), we achieve the final relevant pixel map, shown in \autoref{fig:irrelevant-pixels-example}b.
% We count this number for the three datasets, finding that the average COCO image's ground truth labels comprise X\% of the pixels; MOT Challenge labels comprise an average Y\% of the pixels, and PASCAL VOC labels comprise an average Z\%. This suggests that CNNs can save significant compute resources by ignoring irrelevant pixels.

Ground truth pixels alone do not represent all relevant pixels. A typical CNN uses not only the pixels comprising the object, but also the \textit{pixels from the surrounding area of an object} to extract features that contextualize and understand the object~\cite{zhang_object_2019, gauen_comparison_2017}.

% \diff{Simply counting the number of ground truth pixels in a dataset is trivial, but would not be a realistic estimation of all relevant pixels.}   These contextual pixels need to somehow be included in our estimate of relevant pixels.

To properly include contextual pixels that surround ground truth, we devise a method that uses \textit{depth maps}. Shown in \autoref{fig:depth-map-example}, an image's depth map represents each pixel in the image with one value, referred to as the pixel's \textit{depth level}, denoting how far away from the camera that pixel is.

\begin{figure}[b]
    \centering
    \subfloat[]{
        \includegraphics[width=0.47\linewidth]{figures/depth_map_example.jpg}
    }
    \subfloat[]{
        \includegraphics[width=0.47\linewidth]{figures/ground_truth.jpg}
    }
    \caption{\diff{Depth maps can show regions of contextually related pixels. The ground truth labels indicate which of those regions would count as relevant.} \textbf{(a)} Example of a depth map (for the image in \autoref{fig:irrelevant-pixels-example}). White pixels represent objects that are closer to the camera (shallower depth level) while darker pixels represent objects that are further from the camera (deeper depth level). \textbf{(b)} \diff{Ground truth label for the image, used to identify relevant pixels.} One can see that pixels at the same depth level as an object tend to be contextually related (\diff{a chunk} of the road, in this case) and are useful for CNNs.}
    \label{fig:depth-map-example}
\end{figure}

% \todo[inline]{Figure 2 shows the ground as light gray but Figure 1 says the ground is irrelevant. Why?}

Pixels that have similar depth levels to a given object \diff{on the ground} are known to provide useful, contextual pixels that surround the object~\cite{song_semantic_2017}. For example, a car will be at a similar depth level as the road on which it drives. A seated person, the person's chair, and a region of the floor would be at similar depth levels. Put another way, given a ground truth object label in an image, we need to find all the other pixels at a similar depth level to the object in order to capture all relevant pixels. The other pixels can then be discarded as irrelevant. 
% \todo[inline]{Abhi: Are there any other examples of this definition holding true? Will birds and the sky be at the same depth level?}

Most popular computer vision datasets (including the three examined by this paper) contain images taken with single-lens cameras. Monocular depth estimation techniques are used to generate depth maps on such images~\cite{khan_review_2021}. In this paper, we use ``MiDaS,'' a depth estimation model by Ranftl, et al.~\cite{ranftl_towards_2020} MiDaS is chosen because it uniquely trained using a mix of diverse datasets, dramatically improving its performance on Microsoft COCO, our largest target dataset.

\diff{To count the number of irrelevant pixels in a dataset image, we augment ground truth pixels with depth-mapped pixels, as described in in \autoref{fig:counting_irrelevant_pixels}}. We run MiDaS on the image, generating a depth map. We then overlay the image's ground truth on the depth map to register the ground truth depth levels. Finally, we mark all pixels at those depth levels as ``relevant'' and all the remaining pixels as ``irrelevant.'' This creates a binary, pixelwise map that indicates whether a pixel is relevant or not. The relevant pixels then fully enclose the ground truth, as well as related, contextual pixels (such as a chunk of the road in \autoref{fig:counting_irrelevant_pixels}).

% \todo[inline]{YHL: I do not follow the logic. Do you need the ground truth to find irrelevant pixels? If you already have ground truth, why do you need to run CNN for computer vision?}

% \todo[inline]{VC: The idea of using depth independently is not clear. If you have ground truth, you can show the focus convolution to be effective. By using depth you are increasing the size of the foreground and thus increasing computations. If you can show that you can use depth map only to get a binary relevant/irrelevant area albeit it being always bigger that is fine. You can compare the savings with depth only and with ground truth (which would be limit for good performance). }

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/counting_irrelevant_pixels.jpg}
    \caption{\diff{Proposed method for counting the number of irrelevant pixels that exist in datasets, using depth maps and ground truth.} First, use MiDaS to generate a depth map for the image. Next, find the depth level corresponding to the pixels in the ground truth label as Depth Level X. Finally, create a binary, pixelwise mask where all pixels at Depth Level X are considered relevant, while all other pixels are irrelevant. }
    \label{fig:counting_irrelevant_pixels}
\end{figure}


% \todo[inline]{Figure 3 has a problem: If you already have ground truth, why do you need to run computer vision?}
% \todo[inline]{Abhi: I agree with this comment. Why can't I use the following $\frac{\text{# pixels in ground truth bounding box}}{\text{# pixels in image}}?$ Upon re-reading I understood that your definition of ``relevant'' is anything at the same depth (or closer) than the objects within bounding boxes. Is that correct? Could you justify that definition in a line or two?}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figures/dataset_relevant.jpg}
    % \subfloat[]{
    %     \includegraphics[width=0.3\linewidth]{figures/pascal_relevant.jpg}
    % }
    % \subfloat[]{
    %     \includegraphics[width=0.3\linewidth]{figures/mot_relevant.jpg}
    % }
    % \subfloat[]{
    %     \includegraphics[width=0.3\linewidth]{figures/coco_relevant.jpg}
    % }
    \caption{Average percentage of pixels that are relevant in the three datasets. As shown, most images contain 50\%-60\% relevant (40-50\% irrelevant pixels). This means that in most images, 40-50\% of pixels do not contribute to useful CNN computations.}
    \label{fig:distribution-irrelevant-pixels}
\end{figure*}

\begin{figure*}
    \centering
    \subfloat[]{
        \includegraphics[width=0.19\linewidth]{figures/depth_level_chart.jpg}
    }
    \subfloat[]{
        \includegraphics[width=0.24\linewidth]{figures/pascal_depth_pie.jpg}
    }
    \subfloat[]{
        \includegraphics[width=0.24\linewidth]{figures/mot_depth_pie.jpg}
    }
    \subfloat[]{
        \includegraphics[width=0.24\linewidth]{figures/coco_depth_pie.jpg}
    }
    \caption{\diff{In the three datasets, objects are largely found in a specific subset of contiguous depth levels. This suggests that depending on the computer vision application, some depth levels are more relevant than others.} \textbf{(a)} Depth level legend. Lighter colors are shallower, darker colors are deeper. \textbf{(b)} PASCAL VOC. The majority of objects (38\%+27\%=65\%) are located in depth levels 0.2-0.6. \textbf{(c)} MOTChallenge. The majority of objects (30\%+27\%=57\%) are are located in depth levels 0.4-0.8. \textbf{(d)} COCO. Like PASCAL VOC, a large majority of objects (31\%+34\%=65\%) are distributed in depth levels 0.2-0.6.}
    \label{fig:depth_level_observations}
\end{figure*}

% \todo[inline]{Abhi: Is it possible for the colors in the pie charts to appear in the same order as the legend? Right now in Fig. 5(b), when looking clock-wise, we have 13\% for 0.0-0.2, then 18\% for 0.6-0.8, then 38\% for 0.2-0.4, then 27\% for 0.4-0.6, and finally 4\% for 0.8-1.0.}

% \todo[inline]{Abhi: why is there a black bar at the bottom of the last image in Fig. 3? Shouldn't that portion also be relevant?}
% \todo[inline]{Figure 4 can be merged into a single bar graph using three gray levels and percentages.}

\subsection{Exploring Datasets for Irrelevant Pixels}
\label{subsec:exploring_datasets_for_irrelevants_pixels}
We use our method to count irrelevant pixels in each image in the three datasets, totaling nearly 200,000 images. Results are shown in \autoref{fig:distribution-irrelevant-pixels}. Irrelevant pixels are quite common in the three datasets. On average, 42\% of all pixels are irrelevant in PASCAL VOC, 49\% are irrelevant in MOT Challenge, and 45\% are irrelevant in COCO. This suggests that CNNs are wasting significant amounts of compute resources on embedded devices by computing convolutions on all those irrelevant pixels.

These results are consistent with a sanity check on other dataset and general photography studies. Images that are center-framed and 2/3-framed (a popular way for photographers to frame their shots) tend to place subjects in about 40\%-70\% the image, leaving 30\%-60\% of the image as empty space or background~\cite{jin_aesthetic_2012}. In addition, a previous study of other datasets found that human subjects tended to be sized between 39\%-67\% of the image~\cite{gauen_comparison_2017}, leaving 33\%-61\% empty space. Assuming a rough equivalence between empty space and irrelevant pixels, the distribution of \autoref{fig:distribution-irrelevant-pixels} appears to follow both of these trends.

\diff{Although exploring fully automated techniques for identifying irrelevant pixels at inference time (without the use of ground truth) is outside the scope of this short paper, we make an observation that can guide efforts in this area. \textit{We observe that these datasets tend to contain relevant objects around the same depth levels.}}
% \todo[inline]{Abhi: I don't know if we can make this claim. It reads like you are saying that, when looking at the relevant pixels of busses (i.e., the bus itself and the road and the other pixels at a similar depth), we find many \textit{other} objects (e.g., pedestrians, cars, bikes, etc.). The paper does not describe an experiment to validate this. Are we doing an experiment that finds all \textit{relevant} pixels, and then checks how many ground-truth bounding boxes are within this \textit{relevant-region}?}
% \todo[inline]{VC: Agree with Abhi's remark.}
\autoref{fig:depth_level_observations} shows that on average, objects tend to be closer to the camera (shallower depth level) for both PASCAL VOC and COCO, and further away from the camera (deeper depth level) for the MOTChallenge. This suggests that an automated irrelevant pixel identification system could use depth mapping to only focus on pixels from specific depth levels, without needing to know ground truth information. For example, a surveillance camera might be able to automatically discard long-distance pixels.

% \todo[inline]{It is not obvious Figure 5 is necessary.}

% \todo[inline]{Abhi: Fig 4 and Fig 5 are showing similar information? One can be excluded, in my opinion.}

% \section{For Somto}
% \subsection{Summary of state-of-the-art in single-camera depth estimation}


% DORN(Deep Ordinal Regression Network for Monocular Depth Estimation), a current state-of-the-art method for depth estimation utilizes a supervised framework to estimate depth maps. The method used to estimate depth  involves a dense feature extractor, space-increasing discretization(SID) strategy, cross channel information learner, multi-scale feature learner, encoder, and ordinal regression optimizer to achieve high accuracy and high quality depth estimation, while avoiding unnecessary spatial pooling which leads to faster convergence.~\cite{DORN Fu et al.}


% \subsection{What is MiDaS, and why we picked it}
% MiDaS is a modern machine learning model for monocular depth estimation which can be trained on a diverse number of datasets. We picked it because of its versatility and ability to produce image depth maps on a diverse dataset of images. The challenges which other image depth maps estimation methods face is the reliance on acquiring a large and diverse training set which cover a variety of different enviroments across different scales. Due to this limitation, bias  often emerges in the models. Therefore, although other depth estimation methods could deliver state-of-the-art results, they are not able to deliver state-of-the-art results across a variety of different environments.  

% We picked Midas because Midas does not suffer from this limitation of diverse datasets. Midas avoids this bias by using methods which allow for training the model with a mix of multiple datasets regardless of their incompatible annotations.The Midas Loss function is able to account for the differences that would occur in different datasets. Midas uses scale and shift-invariant losses to handle the ambiguities which exist across different datasets due to difference in scale and other disparities.\cite{Midas Ranftl et al.} This thus allows Midas to combine datasets from different sources and feed the model during training. This superb generalization is the main reason which Midas was able to outperform prior state-of-the-art for monocular depth estimation on an evaluation across six different datasets~\cite{Midas Ranftl et al.}





